ClutterGen: A Cluttered Scene Generator for Robot Learning

We introduce ClutterGen, a physically compliant simulation scene generator capable of producing highly diverse, cluttered, and stable scenes for robot learning. Generating such scenes is challenging as each object must adhere to physical laws like gravity and collision. As the number of objects increases, finding valid poses becomes more difficult, necessitating significant human engineering effort, which limits the diversity of the scenes. To overcome these challenges, we propose a reinforcement learning method that can be trained with physics-based reward signals provided by the simulator. Our experiments demonstrate that ClutterGen can generate cluttered object layouts with up to ten objects on confined table surfaces. Additionally, our policy design explicitly encourages the diversity of the generated scenes for open-ended generation. Our real-world robot results show that ClutterGen can be directly used for clutter rearrangement and stable placement policy training.

==> rebuttals/rebuttal_4LKe_2.tex <==
\appendsection{Reviewer 4LKe}

We appreciate the reviewer's detailed examination and discussion of our paper. We will address the reviewer's concerns in the following response points:

\begin{myquote}
\textit{\small``While the efficiency comparison is already compelling, it would be even more convincing to show that an equivalent dataset size ClutterGen-200 can either match or even outperform the human-curated equivalent dataset Human-200."}
\end{myquote}

We thank the reviewer for this suggestion. We have conducted a comparison between ClutterGen-200 (0.50) and Human-200 (0.52). As the original comparison indicated, ClutterGen can create diverse and effective training data in under one minute, whereas a human expert needs 1.5 hours to create a dataset that is only 4\% of its size. The new comparison shows that even if ClutterGen is given 200 data points, we can still perform on par with the Human-200. Hence, our conclusion still holds.

\begin{myquote}
\textit{\small``It is suggested that ClutterGen can be applied iteratively to construct a scene graph, e.g.: "fork on top of plate on top of table". It would be powerful to showcase an example of this or something equivalent as a proof-of-concept to show how ClutterGen can fully populate a given scene (e.g.: setting a dinner table)."}
\end{myquote}

As discussed in Section 4.2., a simple semantically meaningful setup can be achieved by controlling the queried region. For instance, here we show that we can generate a scenario where ``a laptop is placed on the book or a globe is placed next to it, etc." by controlling the queried region. We leave more complex semantically meaningful scene generation as future work.

\begin{myquote}
\textit{\small``I was surprised to see no comparison with a "smarter" rejection sampling technique -- e.g.: in simulation (and presumably in real, given ground-truth object meshes), given a proposed placement pose collision information should be already be known. This coupled with object bounding box information should allow rapid rejection sampling without having to actually step physics many times. Other than speed improvements, what additional key benefits does ClutterGen have over such an approach?"}
\end{myquote}

ClutterGen allows more complex object relationships, such as stacking on top of others. Some qualitative results can be seen in Fig. 1(b). In such cases, stable poses can't be easily computed using object-bounding boxes due to uneven contact surfaces between objects with complex geometries. Fing stable placements therefore require an implicit understanding of object dynamics and contacts. ClutterGen learns such implicit knowledge through iterative refinement based on the simulator feedback.

Moreover, as mentioned in Line 150, our random rejection sampling did involve heuristic computation that pre-computes the z-axis pose based on object and scene bounding boxes. However, success rates remain low due to clutter requirements.

\begin{myquote}
\textit{\small``How were the different dataset groups selected? Were they all randomly selected or was there some semantic / geometric distinction (e.g: "all kitchen items" or "all convex items", etc.)"}
\end{myquote}

The object datasets are manually selected based on semantic distinctions. For example, group 1 is the dining table group, group 2 is the study table group, group 3 is the office group, group 4 is the kitchen group, and group 5 is the real object group mostly from kitchen. We also provided the visualization of these objects in Appendix Fig. 11. We will add this information into the Appendix as well.

\begin{myquote}
\textit{\small``One interesting qualitative trait of the learned placement policy is that it appears it is biased towards placing objects towards the edges of the supporting surface (as Fig. 5 also quantitatively shows). Could this possibly bias results and result in object placement distributions that don't necessarily align with "natural" distributions found in the real world? ``}
\end{myquote}

Our task requires placing ten objects within a narrow space under strict stability conditions, which is quite challenging. To complete the scene (i.e., place all 10 objects), ClutterGen learns to allocate space for the remaining objects. Thus, it intuitively places objects along the edge to avoid collisions, hence introducing potential biases. However, this bias can be mitigated by shrinking and rotating the queried region, as shown in Section 4.2, to create more "natural" distributions. Using a larger table or placing fewer objects will also mitigate this behavior.

\begin{myquote}
\textit{\small``I also wonder if this is in part due to the fact that the policy only observes the current set of already-placed objects and the current queried object instead of the full set of future objects to be placed, leading the policy to avoid placing objects in the center because it limits the possibility for future (unknown) objects to be placed. I am curious to hear the author's thoughts on this or if they have considered this alternative setup!"}
\end{myquote}

We thank the reviewer for this great idea. We believe that having ClutterGen to observe future objects can help encourage the algorithm to consider the full arrangement of all objects. In our setting, due to our RL formulation, each policy has seen all objects during training in a randomized order. Therefore, the policy should have the knoweldge about all the objects, which is similar to what the reviewer is suggesting. We leave the comparison between these two implementations as future work.

\begin{myquote}
\textit{\small``Can the method be applied to non-rectangular surfaces, e.g.: a circular or abnormally-shaped table?"}
\end{myquote}

Yes, we have included multiple examples in Fig.1(b), and the discussion of this experiment is included in Section 4.2

\begin{myquote}
\textit{\small``It seemed surprising that the placement policy suffered when the sampling surface was translated (Sec. 4.2). Assuming that the entire surface is still sampleable, I would expect the same placements to be valid. Has any sort of normalization with respect to the sampling surface been considered to prevent overfitting?"}
\end{myquote}

Different queried regions or queried scenes will introduce different placement strategies. 
Therefore, we do not normalize the dimension of the region or the scene. We would like to clarify that our results in Section 4.2 are a zero-shot generalization test to different queried regions desipte the original training does not randomize the queried region. Therefore, a drop in the zero-shot generalization test actually provides evidence that our method is not heavily overfitting and can potentially handle various queried surfaces if we further randomize the queried regions during training.

\begin{myquote}
\textit{\small``What is the role of the human selecting the preferred setup for the object rearrangement task? It seems that this would mainly allow the user to select setups that are "easier" to achieve for the robot compared to other alternative proposals."}
\end{myquote}

We would like to clarify that the goal for human selection is not to select setups that are easier to achieve for robots. Since ClutterGen can generate multiple proposals of the scene layouts, we provide this human selection interface to demonstrate that our setting allows the users to select among these proposals based on their preferences.

\begin{myquote}
\textit{\small``Minor syntax issues:
L147: closet $\rightarrow$ closest
L148: RSS presumably should be RRS"}
\end{myquote}

We thank the reviewer for pointing this out. We will fix these typos in our revised version of the paper.


==> rebuttals/rebuttal_fQzd_1.tex <==
\appendsection{Reviewer fQzd}

We appreciate the reviewer for such a detailed examination and discussion of our paper. We aim to address the reviewer’s concerns with the point of response:

\begin{myquote}
``Quality: The work is generally high quality. The proposed algorithm is clearly explained and its performance is validated through a variety of interesting experiments. However, important experiments where the work is compared to other recent procedural generation tools from the variety of simulator groups like AI2Thor (ProcThor, Holodeck), BEHAVIOR (iGibson, OmniGibson), etc. are missing - currently it is not obvious whether this method performs better, on par with, or worse than those existing approaches with heuristic rules. Tradeoffs should also be discussed." + ``The actual merit of the described approach (e.g. RL for clutter generation) can only be understood when the approach is compared to existing heuristic-based generation methods. Such experiments are not included in the manuscript and thus, it is hard to gauge the significance of the contribution." + ``How does the approach compare against clutter generation heuristics from the SOTA simulators rather than just random placement?"
\end{myquote}

Current simulators mainly use heuristics to ensure the generated object layouts are semantically meaningful but typically do not explicitly handle physical stability. Due to the constrained spaces from the heuristics, current simulators typically step forward for multiple trials until finding a relatively stable scene in a random manner. ClutterGen, on the other hand, focuses on ensuring the generated object layouts are physically stable. Therefore, our method is orthogonal to existing heuristic methods. We believe combining ClutterGen with existing semantic heuristic methods can improve the overall generation to be both physically and semantically meaningful.

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{rebuttals/semantic_rebuttal.pdf}
    \caption{\footnotesize
        \textbf{Generate semantically meaningful setups by controlling the queried region.}
    }
    \label{fig:sem_mean1}
    \vspace{-2mm}
\end{figure}

\begin{myquote}
\textit{\small``The proposed algorithm provides no way of guiding the generation towards semantically-meaningful clutter rather than just physically stable, and in fact probably captures a very small subset of what's physically stable, too. For example, clutter in a kitchen cabinet or fridge will usually have certain important characteristics about it stemming from the distribution of the objects involved and their placement etc. - simply placing random objects in a rejection sampling fashion during training will NOT be a good approximation of this distribution and thus may not be very meaningful to help robots learn to work in such environments." + ``How do you ensure semantic realism (e.g. the kind of clutter we see is actually relevant for work a robot might do in real life)?"}
\end{myquote}

We agree with the reviewer that our current main focus is to generate physically stable and diverse cluttered object layouts. We do believe that our method can be generalized toward semantically meaningful clutter. As discussed in Section 4.2., a simple semantically meaningful setup can be achieved by controlling the queried region. For instance, Fig.~\ref{fig:sem_mean1} shows that we can generate a scenario where ``a laptop is placed on the book or a globe is placed next to it, etc." by controlling the queried region. We leave more complex semantically meaningful scene generation as future work. One possible extension to ClutterGen is to add a semantic reward to our RL formulation in addition to the stability reward.

\begin{myquote}
\textit{\small``The proposed algorithm only performs transformations along one rotational axis. This is a major limitation that keeps its generations from being semantically realistic. Whether or not a good policy can be learned in the full three-axis case remains to be seen."}
\end{myquote}

We agree with the reviewer that an exciting future direction is to move further from our current focus on physically stable and diverse clutter generation to also consider the semantic meaning of the generations. In this case, relaxing the z-axis constraints is definitely necessary. As stated above, one possible way is to add a semantic reward to our RL formulation in addition to the stability reward. We will mention this point in our limitation and future work section in our revised paper.

\begin{myquote}
\textit{\small``How do you ensure the diversity / completeness of the physically stable configurations (e.g. doesn't the model just learn to build the easier physically stable configurations rather than a good sample of the full distribution?)"}
\end{myquote}

We have implemented multiple designs to encourage diversity. First, during training and inference, the order of queried objects is randomized, leading to diverse decision-making. Second, the beta distribution, which can represent more diverse distributions than the normal distribution, is shaped with a relatively large entropy coefficient in the loss function during training. This high entropy promotes diverse placements for each object, introducing diverse scene setups. Finally, as discussed in Section 4.2, the queried region can be randomized through translation and rotation, forming comprehensive distributions during the inference.

==> rebuttals/rebuttal_qZ9R_3.tex <==
\appendsection{Reviewer qZ9R}

We sincerely thank the reviewer for their thorough examination and insightful discussion of our paper. We will address the reviewer's concerns in the following points:

\begin{myquote}
\textit{\small ``One of my primary concerns is that the problem might not be as hard as the authors make it seem. For instance, I didn’t see any example in the video that considered something like object stacking, and this kind of exploration is not encouraged by the model."}
\end{myquote}

We would like to clarify that the complex exploration such as object stacking was indeed handled by our method. For instance, in Fig. 1(b), row 2, column 4, the telephone and keyboard are stacked on top of the notebook and remain stable. Similarly, in Fig. 1(b), row 2, column 6, a mug is stacked on top of a green book. More examples can be found in Fig. 1(b), and we have highlighted this behavior in the last sentence of Section 4.2. Finally, as described in Section 4.2, our scene generation method is highly controllable by adjusting the queried region, making it easy to create desired stacking relationships (e.g., applying the queried region on top of the other placed object). We have also provided the zoomed-in visualization examples and another pre-specified object relationship generation example shown in Fig.~\ref{fig:sem_mean3}. 

\begin{figure}[h!]
    \centering
    \includegraphics[width=0.7\linewidth]{rebuttals/semantic_rebuttal.pdf}
    \caption{\footnotesize
        \textbf{Create setups with complex relationships by controlling the queried region.}
    }
    \label{fig:sem_mean3}
    \vspace{-2mm}
\end{figure}

Moreover, the difficulty of the task can be seen from quantitative evaluations in both Fig.1 (a) and Tab. 1. We would like to highlight that one of our contributions is to recognize the difficulty of this task and provide a strong solution to it, as the problem is essential for scalable robot training.

\begin{myquote}
\textit{\small ``Further, the objects can only be translated and rotated about the z axis, so the envelope of the surface that will touch the table is fixed. Given this setup, it's unclear why objects would just randomly fall like the pitcher in the video if it's placed on a free part of the table. Nothing about the pitcher rotating about its z axis on a flat surface should change its dynamics or stability."}
\end{myquote}

We would like to highlight that the task is more challenging than it appears. Our task involves fully 3D placement, meaning objects can be translated along the x, y, and z axes, as shown in Fig. 4. A bad z-axis pose prediction can place the object in mid-air or insert it into the table, causing it to fall or explode, as shown in the video. Moreover, the z-height of the placement cannot be simply computed using the object's bounding box and table height for two reasons: (1) The bottom surface of the object might not be perfectly flat, such as the fork shown in Fig. 1. (2) The queried object may need to be placed on top of other objects with a non-horizontal pose (e.g., Fig. 1(b), row 2, column 4), where the z pose cannot be easily computed. The proposed solution by the reviewer is captured by our baseline comparison (line 150) where a heuristic is used to compute the position of the supporting surface in the queried scene and randomly places objects within the queried region. However, the success rate is very low and almost zero.

\begin{myquote}
\textit{\small ``Building on my previous comment, it seems like simple baselines could have been used in the evaluation to further motivate the approach. For instance, using a potential field approach to avoid collisions and place objects in free spaces is well-established in robotics and seems like a reasonable baseline. Objects can be guided by repulsive forces from other objects and attractive forces towards the desired position on the table. This method is computationally efficient and intuitive for the problem as described."}
\end{myquote}

The potential field approach does not apply to our task for several reasons:

(1) Our task is to find a physics-compliant stable pose for the queried object, not to plan a collision-free trajectory. The main challenge is finding the desired position in a cluttered environment, where collisions sometimes are acceptable such as stacking.
(2) A well-known weakness of the potential field approach is that it could get stuck in local minima. Our method uses a closed-loop mechanism to iteratively generate accurate, stable poses to avoid local minima.
(3) Our method can generate highly diverse setups without human heuristic efforts. In contrast, the potential field approach may require additional heuristics.

\begin{myquote}
\textit{\small ``Also, treating the problem as a 2D packing problem on the surface in contact with the table could indeed be a simpler and more straightforward approach. This method is extensively studied and has efficient algorithms that could be adapted for the scenario described. Now, to be clear, these baselines would not at all be reasonable if full rotation and object stacking would be involved; however, that is not the case in this version of the paper."}
\end{myquote}

As stated above, our task is to place objects in 3D space rather than 2D, which involves the height of the placements such as stacking. To the best of our knowledge, there have not been successful and widely adopted approaches in 3D bin packing with irregular mesh objects. Such settings require several challenging steps, including bounding volume calculation, sorting, placement, collision detection, orientation adjustment, and optimization. The computation increases significantly as the scene becomes more cluttered and the number of queried objects grows.

\begin{myquote}
\textit{\small ``While the authors emphasize the physical simulation to ensure stability, I was surprised to see ``positive" examples in the video with large parts of objects hanging off the edge of the surface. While the simulator may deem this as ``physically stable", allowing for this just seems impractical and unnecessary. This is, yet again, something that a simpler approach would simply not tolerate and would easily avoid."}
\end{myquote}

Our approach can also easily handle such a scenario if this behavior is not desired. As discussed in Section 4.2, one can shrink the queried region by leaving the margin out to eliminate the hanging-off scenarios.

\begin{myquote}
\textit{\small ``In 3.2: you say ``$orientation \in \mathbb{R}^{4}$". However, assuming you are using four values here to represent a unit quaternion, this will not be the space of $\mathbb{R}^{4}$
, this will instead be a Lie group of unit quaternions, commonly referred to as $\mathbb{H}$."}
\end{myquote}

We will correct this symbol in our revised paper.

\begin{myquote}
\textit{\small ``Provide a stronger justification for why reinforcement learning is necessary for this problem. This could include a discussion of the limitations of simpler methods in the specific context of ClutterGen’s objectives."}
\end{myquote}

Due to the complexity of this problem (though intuitively it appears a simple task) as stated above and in our paper, naive baselines based on heuristics and traditional optimization cannot handle complex geometries, object relationships, and implicit understanding of contact and object dynamics. On the other hand, our closed-loop reinforcement learning formulation aims to leverage the strong expressiveness of neural network-based policy to iteratively place objects under physical stability constraints, while implicitly capturing the above complex factors from the environment feedback. Moreover, due to the lack of ground-truth labels for object layouts, it is challenging to apply supervised learning directly to this problem. We will add these clarifications to our revised paper.

\begin{myquote}
\textit{\small ``Address concerns about the perceived complexity of the problem. Explain why objects might fall in the simulation and how ClutterGen addresses these challenges uniquely compared to simpler methods."}
\end{myquote}

Please refer to our above response on the simple baselines. The object falling can happen when the object z-height is not appropriately chosen which causes the object to be placed in the air or inside the table surface, or collide with the irregular surface of other objects when being stacked.

\begin{myquote}
\textit{\small ``Longer term, I highly recommend incorporating full translations and rotations. Many of my previous concerns would go away."}
\end{myquote}

We agree with the reviewer that a future direction is to allow full rotations. We have also mentioned this in the Limitation section. In particular, full rotations will allow more diverse generations. Our current approach provides a solid foundation for this generalization. We believe our claims that ClutterGen can generate physically stable, diverse, and cluttered object layouts remain the same. We leave the exploration of incorporating full rotations as future work.

